Weak and cyclic amenability for Fourier algebras of connected Lie groups

Using techniques of non-abelian harmonic analysis, we construct an explicit, non-zero cyclic derivation on the Fourier algebra of the real $ax+b$ group. In particular this provides the first proof that this algebra is not weakly amenable. Using the structure theory of Lie groups, we deduce that the Fourier algebras of connected, semisimple Lie groups also support non-zero, cyclic derivations and are likewise not weakly amenable. Our results complement earlier work of Johnson (JLMS, 1994), Plymen (unpublished note) and Forrest--Samei--Spronk (IUMJ 2009). As an additional illustration of our techniques, we construct an explicit, non-zero cyclic derivation on the Fourier algebra of the reduced Heisenberg group, providing the first example of a connected nilpotent group whose Fourier algebra is not weakly amenable.

==> WAAGmac.tex <==
% macros common to arXiv version and submitted version

\NeedsTeXFormat{LaTeX2e}
\RequirePackage{amsmath,amssymb,amsfonts}
\numberwithin{equation}{section}


%------------


\RequirePackage{amsthm}   %Inbuilt environments for defns etc
%\usepackage{theorem}

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse


%Styles for theorems, definitions, remarks

\newcommand{\thf}{\sc} % alias for theorem heading font

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem*{thmstar}{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
\newtheorem*{notn}{\thf Notation}
\newtheorem{eg}[pulse]{\thf Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}
\newtheorem*{remstar}{\thf Remark}


\renewcommand{\emph}[1]{{\sl #1}\/} % use slanted font for emphasis
%\newcommand{\st}{\;:\;}
\newcommand{\defeq}{:=}
\newcommand{\sid}{\operatorname{\sf id}}  % generic notation for identity map

% Abs value, norm
\newcommand{\abs}[1]{\vert{#1}\vert}
%\newcommand{\Abs}[1]{\left\vert{#1}\right\vert}
\newcommand{\norm}[1]{\Vert{#1}\Vert}
%\newcommand{\Norm}[1]{\left\Vert{#1}\right\Vert}

\newcommand{\lin}{\operatorname{lin}}

% inner products
%\newcommand{\ip}[3][]{\langle{#2},\,{#3}\rangle_{#1}}
\newcommand{\ip}[2]{\langle{#1},\,{#2}\rangle}
\newcommand{\Dom}{\operatorname{Dom}} % domain of an unbounded operator.

% Fourier algebra, etc
\newcommand{\FA}{\operatorname{A}}
\newcommand{\FS}{\operatorname{B}}
\newcommand{\VN}{\operatorname{VN}}
\newcommand{\Cst}{\operatorname{C}^*}

% Various generic letters in different fonts
%% calligraphic
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
%% sans-serif
\newcommand{\sF}{{\sf F}}
\newcommand{\sH}{{\sf H}}
\newcommand{\sM}{{\sf M}}

%% abbreviations for Greek letters
\newcommand{\lm}{\lambda}


%--------------------------------------------


% journals seem to want upright roman numerals in numbered lists, we need to force this if in an italic environment
\newenvironment{newnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}

\newcommand{\twomat}[4]{{\begin{pmatrix} #1 & #2 \\ #3 & #4     \end{pmatrix}}}
   
%%Personal preference and fundamentals
\newcommand{\veps}{\varepsilon}
\newcommand{\wtild}{\widetilde}
\newcommand{\what}{\widehat}
\newcommand{\blob}{\bullet}
\newcommand{\blank}{\underline{\quad}}
\newcommand{\iso}{\cong}
\renewcommand{\Re}{\operatorname{\sf Re}}
\renewcommand{\Im}{\operatorname{\sf Im}}
%\DeclareMathOperator{\op}{op}
\newcommand{\id}[1][]{{\sf 1}_{#1}} % identity of group, algebra, object in category
\newcommand{\wstar}{\ensuremath{{\rm w}^*}}

\newcommand{\tr}{\operatorname{Tr}} % matrix trace
\newcommand{\Tr}{\operatorname{Tr}} % matrix trace
\newcommand{\spec}{\operatorname{sp}} % spectrum
\newcommand{\pair}[2]{\langle{#1},\,{#2}\rangle}
\newcommand{\supp}{\operatorname{supp}}

\newcommand{\tp}{\mathbin{\otimes}}



% Special objects (in the Bourbaki sense)
\newcommand{\Cplx}{\mathbb C}
\newcommand{\bbH}{{\mathbb H}} % Heisenberg group
\newcommand{\Nat}{\mathbb N}
\newcommand{\Rat}{\mathbb Q}
\newcommand{\Real}{\mathbb R}
\newcommand{\Torus}{\mathbb T} %Unit circle
\newcommand{\Zahl}{\mathbb Z}

%(Sub)sets
%\newcommand{\Disc}{\mathbb D} %Open unit disc


%% Core commands for (functional) analysis

% Tensor products etc.
\newcommand{\ptp}{\mathbin{\widehat{\otimes}}} % projective tensor product


% Misc
\newcommand{\clin}{\overline{\rm lin}} %closed linear span
\newcommand{\Ind}{{\rm Ind}} %induced representation

%-Banach spaces
\newcommand{\Bdd}{{\mathcal B}}

%% Various Lie groups (group schemes?)
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\OO}{\operatorname{O}}
\newcommand{\SOTHREE}{\SO(3)} % idea is that we can always change our convention/abbreviation if we need to
\newcommand{\SUTWO}{\SU(2)} % idea is that we can always change our convention/abbreviation if we need to

% some function spaces
\newcommand{\ccinf}{C_c^\infty}
\newcommand{\cc}{C_c}

% ad hoc
\newcommand{\Trig}{\operatorname{Trig}}
\newcommand{\eith}{e^{i\theta}}
\newcommand{\sch}{{\sf Sch}} % Schr\"odinger reps
\newcommand{\bmat}{\left(\begin{matrix}}
\newcommand{\emat}{\end{matrix}\right)}

% for ax+b
\newcommand{\Psibar}{\overline{\Psi}}

\newcommand{\madb}{\mathop{{\rm M}_a\partial_b}}

\newcommand{\dom}{\operatorname{dom}} % domain of unbounded operator
%\newcommand{\dd}{\operatorname{\mathbf d}}
\newcommand{\dd}{\partial}

\newcommand{\bh}{{\bf h}}

\newcommand{\xnorm}[1]{\norm{#1}_M}
\newcommand{\STN}{{\sf S}} % Schatten class operators


% function spaces associated to Heisenberg group
\newcommand{\SH}{{\mathcal S}(\bbH)} % Schwartz space of Heisenberg group

\newcommand{\hrdual}{\widehat{\bbH}_r}  % reduced unitary dual of $\bbH$.
\newcommand{\Hdual}[1]{L^{#1}(\Real^*, \STN_{#1}, |t|dt)} % Our representation of the NC-L^{#1} space of VN of the Heisenberg
\renewcommand{\Hdual}[1]{L^{#1}(\hrdual, \STN_{#1})}

\newcommand{\dualM}{\widehat{\sf M}}


\newcommand{\cJ}{{\mathcal J}} % notation for L^1\cap L^2
%\newcommand{\cU}{{\mathcal U}} % unitary group

%\newcommand{\bbH}{{\mathbb H}} % 3-dim Heisenberg group

%\newcommand{\Tr}{\operatorname{Tr}}

\newcommand{\stp}{\overline{\otimes}}

\newcommand{\twist}[3]{{#2}\mathbin{\odot}_{#1}{#3}}
\newcommand{\opconv}{\mathbin{\sharp}}

\newcommand{\tnorm}[1]{{\Vert#1\Vert}_{(1)}}
\newcommand{\esssup}{\operatorname{ess.sup}}


% stuff for Lie algebras and Lie groups
\newcommand{\lie}[1]{{\sf #1}}
\newcommand{\fa}{\lie{a}}
\newcommand{\fg}{\lie{g}}
\newcommand{\fh}{\lie{h}}
\newcommand{\fk}{\lie{k}}
\newcommand{\fn}{\lie{n}}
\newcommand{\fr}{\lie{r}}
\newcommand{\fs}{\lie{s}}
\newcommand{\fsl}{\lie{sl}}
\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Ad}{\operatorname{Ad}}
\newcommand{\rad}{\operatorname{rad}}


